Proactive Certificate Validation for VANETs

Security and privacy in Vehicular Ad-hoc Networks (VANETs) mandates use of short-lived credentials (pseudonyms) and cryptographic key pairs. This implies significant computational overhead for vehicles, needing to validate often numerous such pseudonyms within a short period. To alleviate such a bottleneck that could even place vehicle safety at risk, we propose a proactive pseudonym validation approach based on Bloom Filters (BFs). We show that our scheme could liberate computational resources for other (safety- and time-critical) operations with reasonable communication overhead without compromising security and privacy.

==> sections/preliminary.tex <==
\section{Preliminaries}
\label{sec:preliminary}



\subsection{Bloom filter and Counting Bloom Filter}


\textbf{Bloom Filter:} \ac{BF} is widely used for efficient membership checking in Internet applications (e.g., websites~\cite{}, ). Instead of publishing the whole database. A \ac{BF} is built based on the elements in the data set. The \ac{BF} can be published and be used by any node to check whether an element is included in the set or not. Each element in the set are hashed $k$ times, while the output of each hash function is a position in a $m$ bit vector. While an element is inserted into the \ac{BF}, $k$ positions from $k$ hash functions are set to 1 for each item. However, if any of them have already been set to 1 during the insertions of previous items, them bits are simply kept as 1 and ignored. In case the membership of an element needs to be tested, the element is hashes with $k$ hash functions, and $k$ positions from the hash functions are checked with the \ac{BF}. If all $k$ positions were set to 1 in the \ac{BF}, then the element has passed the membership checking. However, \ac{BF} could exhibit false positive rate: it is possible that an element was not included in the set, but all $k$ positions in the \ac{BF} are 1.

\textbf{Counting Bloom Filter:} Another issue of the \ac{BF} is that it does not allow deletion of elements from the \ac{BF}, since a bit in the \ac{BF} might be needed by multiple elements for membership checking: if the bits for an element are set to 0 while deleting it, then it could fail the tests of other elements which also needs the same bits. Counting \ac{BF} maintains a counter for each bit, indicating how many times it has been set 1 by the items. Therefore, when an element needs to be deleted from the \ac{BF}, for each of $k$ positions, the counter is decreased by 1. If the counter of a bit is decreased to 0, then the corresponding bit in the \ac{BF} is also set to 0. For practical reasons, in resource-constrained situation, a counter could occupy a limited memory. For example, if a counter occupy 4 bits, the maximum number the counter could keep is 15. This could result in false negative while counter overflows~\cite{broder2004network}. However, it is not an issue in our scheme, since the counters for the \ac{BF} are only maintained the in the \ac{PCA}, and a traditional \ac{BF} (i.e., without counters) are published to the nodes. We further explain it in Sec.~\ref{sec:scheme}.


\textbf{Bloom Filter Delta:} \ac{BF}-delta is used when the \ac{BF} needs to be updated while a little portion of the elements are changed (e.g., added or deleted). This provide a way to efficiently publish the different between the old and new \ac{BF} with minimum overhead. In our scheme, the \ac{BF}-delta could be used to update revoked pseudonyms and new pseudonyms for the vehicles from another domain.

\textbf{Comparison with Hash:} An alternative to the \ac{BF} would be the concatenation of hash values of the items. Hash values of the elements in the dataset can be concatenated and published as a hash list. In order to check whether an element is included in the dataset, the hash value of the data should be computed and searched in the hash list. 


%\subsection{Merkle Tree Integration}
%As described earlier, \ac{BF} exhibits false positive rate, i.e., an element that does not exist could be falsely identified as a member of a \ac{BF}. This can be utilized by the attacker to insert a false \ac{POI} to mislead a user. In~\cite{ren2009multi}, Merkle tree has been integrated with \ac{BF} to decrease false positive rate while trading off communication overhead. In our scheme, each element is inserted into the \ac{BF}, while we note that the some of the information is always sent together (e.g., restaurants that close to each other). A merkle tree can be constructed from multiple \ac{POI} items, and the root of the merkle tree can be inserted into the \ac{BF}. This decrease the number of elements in a \ac{BF}, while supporting the same amount of \ac{POI} items, resulting in the decrease of false positive rate.

\subsection{Pseudonym Filling Strategy}

Pseudonyms are used to guarantee vehicles' normal operations in the system. Each pseudonym has a limited lifetime and the pseudonyms need to be changed over time while vehicles are operating in the system. Standardization bodies and organizations such as C2C-CC and CAMP, and European projects such as PRESERVE and SeVeCom have been considered preloading of pseudonyms.

Preloading pseudonyms to \acp{OBU} avoid frequent communication with \ac{VPKI} to request pseudonyms. The pseudonyms are issued for an \ac{OBU} for a long period (e.g., 1 year) with overlapping (e.g., C2C-CC, CAMP and PRESERVE)or non-overlapping lifetimes (SeVeCom and Safety Pilot).


\begin{comment}
\textbf{On-demand:} Pseudonyms can be requested on-demand when a vehicle wish to start its trip. In this case, the vehicle request a set of pseudonyms, use them until they expire, and request a new set of pseudonyms. This process is continued until the trip is over. This policy is used to avoid over-provision of pseudonyms to the vehicles. Thus, less pseudonyms would be left expired while they are not used.
\end{comment}

%\textbf{Preloading:}

==> sections/related.tex <==
\section{Related Work}


